ImPress: Securing DRAM Against Data-Disturbance Errors via Implicit Row-Press Mitigation

DRAM cells are susceptible to Data-Disturbance Errors (DDE), which can be exploited by an attacker to compromise system security. Rowhammer is a well-known DDE vulnerability that occurs when a row is repeatedly activated. Rowhammer can be mitigated by tracking aggressor rows inside DRAM (in-DRAM) or at the Memory Controller (MC). Row-Press (RP) is a new DDE vulnerability that occurs when a row is kept open for a long time. RP significantly reduces the number of activations required to induce an error, thus breaking existing RH solutions. Prior work on Explicit Row-Press mitigation, ExPress, requires the memory controller to limit the maximum row-open-time, and redesign existing Rowhammer solutions with reduced Rowhammer threshold. Unfortunately, ExPress incurs significant performance and storage overheads, and being a memory controller-based solution, it is incompatible with in-DRAM trackers. In this paper, we propose Implicit Row-Press mitigation (ImPress), which does not restrict row-open-time, is compatible with memory controller-based and in-DRAM solutions and does not reduce the tolerated Rowhammer threshold. ImPress treats a row open for a specified time as equivalent to an activation. We design ImPress by developing a Unified Charge-Loss Model, which combines the net effect of both Rowhammer and Row-Press for arbitrary patterns. We analyze both controller-based (Graphene and PARA) and in-DRAM trackers (Mithril and MINT). We show that ImPress makes Rowhammer solutions resilient to Row-Press transparently, without affecting the Rowhammer threshold.

==> 7.rfm.tex <==


\newpage
\section{Scaling to Lower Thresholds with RFM}
\label{sec:RFM}



\subsection{Refresh Management (RFM)} 

RFM enables the memory controller to issue additional mitigations (RFM commands) to the DRAM when the activations per bank crosses a threshold. 
However, the actual row to be mitigated still depends on the in-DRAM tracker. The memory controller maintains a {\em Rolling Accumulation of ACTs (RAA)} counter ~\cite{kim2022mithril}) per bank. When any RAA counter crosses a threshold, $RFM_{TH}$, the memory controller resets the RAA counter and issues an RFM to the corresponding DRAM bank.



==> hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
  %\author{\normalsize{ISCA 2024 Submission\textbf{\#\iscasubmissionnumber} -- Confidential Draft -- Do NOT Distribute!!}}

    %\IEEEauthorblockN{\normalsize{ISCA 2024 Submission\textbf{\#\iscasubmissionnumber{}}} -- Confidential Draft --  Do NOT Distribute!!}

%    \vspace{-0.35 in}
    \IEEEauthorblockN{\normalsize{ISCA 2024 Submission\textbf{\#\iscasubmissionnumber{}}} -- Confidential Draft --  Do NOT Distribute!!}
 %   \IEEEauthorblockN{\normalsize{Aamer Jaleel \hspace{5mm} Gururaj Saileshwar \hspace{5mm}Stephen W. Keckler \hspace{5mm}Moinuddin K. Qureshi}}
 %   \vspace{-0.4 in}
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{18cm}{\centering PLEASE DO NOT DISTRIBUTE -- In Submission to International Symposium on Computer Architecture (ISCA) 2024}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}


